Learning Joint ID-Textual Representation for ID-Preserving Image Synthesis

We propose a novel framework for ID-preserving generation using a multi-modal encoding strategy rather than injecting identity features via adapters into pre-trained models. Our method treats identity and text as a unified conditioning input. To achieve this, we introduce FaceCLIP, a multi-modal encoder that learns a joint embedding space for both identity and textual semantics. Given a reference face and a text prompt, FaceCLIP produces a unified representation that encodes both identity and text, which conditions a base diffusion model to generate images that are identity-consistent and text-aligned. We also present a multi-modal alignment algorithm to train FaceCLIP, using a loss that aligns its joint representation with face, text, and image embedding spaces. We then build FaceCLIP-SDXL, an ID-preserving image synthesis pipeline by integrating FaceCLIP with Stable Diffusion XL (SDXL). Compared to prior methods, FaceCLIP-SDXL enables photorealistic portrait generation with better identity preservation and textual relevance. Extensive experiments demonstrate its quantitative and qualitative superiority.

==> sections/introduction_old.tex <==
\section{Introduction}
\noindent
% Recent advancements in text-to-image (T2I) diffusion models \cite{nichol2021glide,ramesh2022hierarchical,rombach2022high,saharia2022photorealistic} have significantly enhanced image generation quality and versatility. A key focus of these developments is personalized generation, which aims to preserve subject identity (ID) from reference images while enabling flexible modifications of other visual attributes.
Recent advancements in text-to-image (T2I) diffusion models \cite{nichol2021glide,ramesh2022hierarchical,rombach2022high,saharia2022photorealistic} have substantially improved the quality and flexibility of image generation. A central objective in this progress is personalized generation, which seeks to retain the subject’s identity (ID) from reference images while allowing versatile modifications of other visual attributes. \par
\noindent
So far, ID-preserving image synthesis has gone through a revolution from tuning-based methods to tuning-free methods. The tuning-based methods \cite{ruiz2023dreambooth,wei2023elite,hu2022lora,gal2022image} achieve ID-preserving generation by test-time fine-tuning. It fine-tunes a pre-trained generative model using couples of reference images, biasing the model to generate photos with subject identical to the references. Although, these methodd can to some extend provide ID preservation capability with limited semantic editability, they are computationally expensive and poor in real-time processing capability. 
% Existing methods \cite{ye2023ip,wei2023elite,ruiz2023dreambooth,kumari2023multi,hu2022lora,wang2024instantid,guo2025pulid} enable users to adapt pre-trained T2I diffusion models to personalized ID through either test-time fine-tuning or in a zero-shot manner. Tuning-based methods \cite{ruiz2023dreambooth,wei2023elite,hu2022lora,gal2022image} fine-tune pre-trained models using one or more reference images, biasing them toward the specified domain. However, these approaches require thousands of iterations to converge during test time, making them computationally expensive and impractical for real-world applications. 
Alternatively, the tuning-free methods \cite{ye2023ip,shi2024instantbooth,guo2025pulid,wang2024instantid,he2024uniportrait,sara2025ipcompose,qian2024omni,han2024face} provide zero-shot solutions. These methods first extract ID features from reference images using a pre-trained encoder, such as a vision encoder \cite{radford2021learning,qian2024omni,oquab2023dinov2} or a face recognition backbone \cite{deng2019arcface,wang2018cosface,wang2018additive,deng2017marginal}, and inject the ID feature through a trainable adapter module into the intermediate representation of a pre-trained generative model. Trained on domain-specific datasets with annotations of image semantics and subject identity, the adapter learns to adapt ID features with pre-exist semantics information from text to recover face of a reference in the output image. The tuning-free methods provide a zero-shot solution for personalization and ID-preservation. Without relying on test-time optimization, tuning-free methods has very low inference latency while maintaining promising capability of ID preservation, text alignment and image quality. 
%The extracted ID features, combined with user-provided text prompts, are processed by additional neural network (NN) modules integrated into the generative model architecture. The entire model is trained on domain-specific datasets with annotations of image semantics and subject identity, eliminating the need for test-time fine-tuning. Consequently, tuning-free methods offer high efficiency and practical applicability. 
\par
\noindent
Despite the advantages, these methods struggle to generate photorealistic images with consistent identity and text semantics. The diversity of expression, head pose, and gesture is limited. The image style are intended to be CG and subject's skin texture is unreal. The generated face are visually incompatible with other part of the image. These problems are caused by the reconstruction-based training paradigms of existing tuning-free methods \cite{guo2025pulid}. Learning an ID preservation model is regarded as a reconstruction problem. The trainable adapter module is trained to blend the ID feature of a reference face with visual contents indicated by text, and try to recover the target face in the output images. In this case, as the text encoder is fixed, there is limited interaction and adaptation between ID information and textual semantics, which leads to sub-optimal generation performance.
% Under this training paradigms, the adapter module learns to blend the reference face visual contents indicated by the text prompt. Since the base model and text encoder are fixed, there is limited adaptation between ID features and text features to generate visually harmony images. 
% Despite the advantages, these methods struggle to balance subject identity preservation with adherence to textual semantics. ID insertion can degrade text alignment \cite{guo2025pulid,ye2023ip,wang2024instantid}, as models optimized for high ID fidelity often have limited capability to edit facial attributes, orientations, and accessories. In diffusion-based image generation, training an ID preservation module is typically framed as a reconstruction problem, with the target image being the reference image and optimized using diffusion loss. However, existing pairwise training data and workflows may encourage the module to rely on ID-irrelevant information, causing the learned parameters to align too closely with the dataset distribution. As a result, generated images often resemble a near copy-paste of the reference, restricting the model’s ability to seamlessly adapt attributes such as facial features, orientation, lighting, and accessories in response to textual prompts. 
\par
\noindent
In this paper, we resolve the above problem from a new perspective. Inspired by Arc2Face \cite{papantoniou2024arc2face}, we model the distribution of portrait images as a forward probability distribution conditioning on subject's identity and textual semantics. The ID-preserving image generation is regarded as sampling process from this distribution given identity and text conditions. We develop a novel encoder called FaceCLIP, which can simultaneously encode ID features and textual information into a unified representation. This representation preserves discriminative information of both identity and text semantics and can be used as the prior condition in portrait image modeling. We propose a multi-modal alignment algorithm to train FaceCLIP. The encoder is optimized using a multi-modal alignment loss that explicitly aligns its joint representation with the original face embedding space, text embedding space, and image embedding space. Further, we incorporate FaceCLIP with Stable Diffusion XL (SDXL) \cite{podell2023sdxl} to learn the forward probability distribution of portrait images. The extensive experiment shows that, trained with proposed multi-modal alignment loss, FaceCLIP effectively learns a decent embedding space capturing both identity and text information. Moreover, the resulting ID-preserving generative model FaceCLIP-SDXL outputs the existing methods quantitatively and qualitatively. The contributions of this paper are summarized as follows:
% Arc2Face\cite{papantoniou2024arc2face} takes an alternative approach, which aligned face embeddings to the text embedding space and finetuned the entire diffusion model to enable more diverse face image generation conditioned on ID. Our method is inspired by Arc2Face \cite{papantoniou2024arc2face}, a foundation model for high-quality face synthesis. Arc2Face\cite{papantoniou2024arc2face} integrates face embeddings and text prompts using a single Vision Transformer (ViT) to guide the diffusion process. However, as the face embedding overwrites the text embedding,  Arc2Face\cite{papantoniou2024arc2face} is limited to face generation and cannot respond to user-provided descriptions for generation. Building on this work, we introduce FaceCLIP, a novel encoder that seamlessly integrates image, text, and ID information through facial features. With FaceCLIP, we develop diffusion models that inherently support face inputs without requiring additional ID feature injection modules. We hypothesize that this joint encoding approach enhances ID preservation, naturally aligns with prompts, and maintains high image quality.
% In particular, we proposed a Dual Cross-Attention mechanism to allow FaceCLIP to combine text prompts and reference images into a multimodal representation. A novel multimodal alignment training algorithm is further developed to ensure the output representation preserves both identity and text information. Meanwhile, our proposed encoder can be seamlessly integrated into any generative model pipeline, endowing it with subject-driven image generation capabilities. In this paper, we take SDXL as our base model to examine the idea and introduce FaceCLIP-SDXL, an image generation model that integrates FaceCLIP with SDXL. FaceCLIP-SDXL can generate high-quality portrait images based on reference face images and text prompts. 
% Experiments show that our FaceCLIP effectively encodes ID information into a text-image subspace representation without hurting the text-image alignment from a standard CLIP model. We also showed that FaceCLIP-SDXL surpasses state-of-the-art ID preservation methods that are based on SDXL in both ID similarity, prompt alignment, and image quality. The key contributions of this paper are summarized as follows:
% A unified representation that encodes both identity and semantic information can serve as a shared conditioning signal for the generative process. Furthermore, training a generative model with ID preservation can be viewed as learning a standard generative model under a specialized prior. 
% Inspired by \textbf{Arc2Face} \cite{papantoniou2024arc2face}, a foundation model for high-quality face generation, we introduce \textbf{FaceCLIP}, a novel multimodal encoder that preserves identity while enhancing text alignment. Arc2Face integrates face embeddings and text prompts using a single Vision Transformer (ViT) to guide the diffusion process. However, it is limited to simple text prompts and cannot process user-provided descriptions for fine-grained image manipulation. In contrast, \textbf{FaceCLIP} combines text prompts and reference images into a \textbf{joint multimodal representation} using a \textbf{Dual Cross-Attention} mechanism. Furthermore, we propose a \textbf{multimodal alignment training algorithm} to ensure that FaceCLIP’s output faithfully encodes both identity and textual information.
%\textcolor{blue}{However, it is limited to process a fixed text prompt and cannot handle user-provided descriptions for fine-grained image manipulation. In this paper, we propose FaceCLIP, a novel encoder that enables image generation with preserved identity and textual semantics. It combines text prompts and reference images into a multimodal representation using Dual Cross-Attention mechanism. Moreover, we propose a novel multimodal alignment training algorithm to ensure the output representation preserve both identity and text information. Our proposed encoder can be seamlessly integrated into any generative model pipeline, endowing it with subject-driven image generation capabilities. Therefore, we further introduce FaceCLIP-SDXL, an image generation pipeline that integrates FaceCLIP with a pre-trained Stable Diffusion XL model. FaceCLIP-SDXL can generate high-quality portrait images based on input face images (or reference images) and user's text prompts. Experiments shows that our FaceCLIP encoder achieves text-image alignment performance comparable to a standard CLIP text encoder. Additionally, FaceCLIP effectively encodes ID information into a subspace of its output representation, demonstrating its ability to capture both identity and textual semantics. Finally, FaceCLIP-SDXL surpasses existing ID preservation methods, achieving state-of-the-art performance in both ID similarity and text adherence. The key contributions of this paper are summarized as follows:}
% (i) a text embedding space learned by a pre-trained CLIP text encoder, (ii) a face embedding space learned by a pre-trained face recognition model, and (iii) an image embedding space learned by a pre-trained CLIP vision encoder. 
% To assess FaceCLIP’s text encoding capability, we apply it to zero-shot classification tasks, where it achieves performance comparable to a standard CLIP text encoder. Additionally, extensive experiments confirm that FaceCLIP effectively encodes ID information into a subspace of its output representation, demonstrating its ability to capture both identity and textual semantics. To further validate its impact on image synthesis, we introduce FaceCLIP-SDXL, an image generation pipeline that integrates FaceCLIP with a pre-trained Stable Diffusion XL model. Experimental results show that FaceCLIP-SDXL surpasses existing ID preservation methods, achieving state-of-the-art performance in both ID similarity and text adherence. The key contributions of this paper are summarized as follows:
% \begin{itemize}
% \item We develope a novel multimodal encoder called FaceCLIP to ensuring a balance between subject identity preservation and textual semantics. 
% \item We propose multimodal alignment training algorithm for our FaceCLIP encoder to learned a unified representation of identity and text.
% \item  We present an advanced image generation pipeline called FaceCLIP-SDXL that surpasses existing ID preservation methods, achieving state-of-the-art performance in identity similarity and text fidelity.
% \end{itemize}
\begin{itemize}
\item We reviewed the existing reconstruction-based ID-preserving image generation models and re-formulate the ID-preserving generation as a sampling process from a forward distribution learned from massive of portrait images with identity and semantic annotation.
\item We designed a novel encoder (FaceCLIP) that encodes both ID and text information into a unified representation for downstream tasks, e.g. image generation.
\item We developed a multi-modal alignment algorithm to train FaceCLIP encoder, making the output representation preserves discriminative information of identity and text semantics.
\item We demonstrate the benefit of FaceCLIP to ID-preserving generation by incorporating FaceCLIP with SDXL. The extensive experiments show that the proposed FaceCLIP-SDXL achieves a new state-of-art performance in ID preservation capability, text adherence, and image fidelity. 
\end{itemize}




% \begin{figure}
% \caption{An identity-preserved foundation model for portrait image synthesis based on SDXL and proposed FaceCLIP encoder.}
% \end{figure}

==> sections/preliminary.tex <==
\section{Motivation}

\subsection{Conditional Image Synthesis}  
Conditional Image Synthesis (CIS) aims to generate images based on specific input conditions such as class labels, textual descriptions, images, or structural constraints. Formally, the generation process is defined as  
\begin{equation}  
x_0 = \mathcal{G}(\epsilon, c),  
\end{equation}  
where a function \( \mathcal{G} \) maps Gaussian noise \( \epsilon \sim \mathcal{N}(0, 1) \) to an image \( x_0 \) based on condition \( c \). CIS plays a crucial role in applications such as image-to-image translation, text-to-image generation, and data augmentation. The primary challenge lies in ensuring high-quality image realism while preserving semantic consistency with the given conditions. Addressing this requires models that effectively capture dependencies between input conditions and generated images, often leveraging deep generative frameworks such as conditional GANs \cite{zhu2017unpaired,karras2019style} or diffusion models \cite{rombach2022high,saharia2022photorealistic,nichol2021glide}.  

\subsection{Subject-driven Image Synthesis}  
Subject-driven Image Synthesis (SIS) is a specialized form of CIS, where the goal is to generate images featuring a specified subject while maintaining semantic consistency with a given text prompt. Here, the condition \( c \) is decomposed as  
\begin{equation}  
c = \mathcal{H}(c_{\text{text}}, c_{\text{id}}),  
\end{equation}  
where \( \mathcal{H} \) represents a transformation function that integrates textual and identity information. This transformation can be implemented using neural network-based identity (ID) adapters in tuning-free methods or through test-time fine-tuning in tuning-based approaches. The text condition \( c_{\text{text}} \) is extracted using a pre-trained text encoder, such as CLIP  \cite{radford2021learning} or T5 \cite{raffel2020exploring}, while the identity condition \( c_{\text{id}} \) is obtained from a pre-trained vision encoder \cite{radford2021learning,oquab2023dinov2} or recognition backbone \cite{deng2019arcface}. Throughout this paper, we narrow the definition of \( \mathcal{H} \) to refer specifically to an adapter or our proposed FaceCLIP encoder. \par

A key challenge in SIS is the inherent conflict between text and identity conditions. The identity feature often disrupts the semantic attributes specified by the text, primarily due to limitations in current training paradigms and ID adapter designs. Existing training datasets consist of tuples \( (I, C, I_r) \), where \( I \) is the target image, \( C \) is its corresponding caption, and \( I_r \) is a reference image cropped from \( I \). Under the standard diffusion-based training framework, training with these tuples forces the ID adapter to reconstruct the reference image, leading it to rely on ID-irrelevant information rather than generalizing subject identity effectively. Furthermore, current methods for integrating ID adapters with text encoders are suboptimal. Typically, adapted ID features are injected into the base model via cross-attention, where identity and text information are naively combined using simple operations such as addition or concatenation \cite{ye2023ip,wang2024instantid,guo2025pulid,sara2025ipcompose,chen2024anydoor}. The balance between identity and text influence is controlled by a hyperparameter \( \eta \). However, this design treats identity and text as competing signals, without guaranteeing their coherent coexistence before being fed into the generative model.  

\subsection{Joint Identity-Text Encoding}  
In standard text-to-image (T2I) generation, text serves as the sole prior for modeling the conditional image distribution. The text embedding space is learned through standalone tasks such as vision-language pretraining \cite{radford2021learning} or language modeling \cite{raffel2020exploring}. In SIS, however, both text and identity should act as prior conditions. This necessitates the development of specialized encoders and learning strategies to construct a joint identity-text embedding space. A well-learned joint representation can effectively resolve conflicts between identity and text features. By leveraging large-scale multimodal data, this embedding space regularizes generative training, reducing overfitting to ID-irrelevant details while preserving both subject identity and textual semantics.


==> tables/ablation.tex <==
\begin{table*}
\small
\centering
\begin{tabularx}{0.9\textwidth}{@{}l|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c}{Internal-v1} & \multicolumn{3}{c}{Unsplash-50} \\ 
& Face Sim. $\uparrow$ & CLIP-T $\uparrow$  & FID $\downarrow$ & Face Sim. $\uparrow$ & CLIP-T $\uparrow$  & FID $\downarrow$ \\
\midrule
FaceCLIP-SDXL$^{\clubsuit}$ & 0.082 & \textbf{0.359} & 87.1 & 0.093 & \textbf{0.368} & 88.1\\
FaceCLIP-SDXL$^{\spadesuit}$ & \textbf{0.869} & 0.332 & \textbf{86.9} & \textbf{0.866} & 0.329 & \textbf{87.8} \\
\bottomrule
\end{tabularx}
% \vspace{-0.05in}
\caption{Quantitative results of FaceCLIP-SDXL with different training strategies: $\spadesuit$ freezing entire FaceCLIP encoder after pre-training; $\clubsuit$ fine-tuning Fusion Block together with base model after pre-training.}
\label{tab:ablation}
% \vspace{-0.2in}
\end{table*}



==> tables/arc2face.tex <==
\begin{table}[h]
\small
\centering
\begin{tabularx}{0.63\textwidth}{@{}c|cc|cc@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Internal-v1} & \multicolumn{2}{c}{Unsplash-50} \\ 
& Face Sim. $\uparrow$ & FID $\downarrow$ & Face Sim. $\uparrow$ & FID $\downarrow$ \\
\midrule
Arc2Face & 0.914 & 7.313 & 0.897 & 7.624 \\ 
FaceCLIP-SD1.5 & \textbf{0.930} & \textbf{5.823} & \textbf{0.919} & \textbf{6.012} \\
\bottomrule
\end{tabularx}
\vspace{0.1cm}
\caption{Comparing FaceCLIP-SD1.5 with Arc2Face in terms of face synthesis.}
\label{tab:arc2face}
\vspace{-0.4cm}
\end{table}



==> tables/face_verification.tex <==
\begin{table}
\small
\centering
\begin{tabularx}{0.5\textwidth}{@{}lcccc@{}}
\toprule
Model & IJBC5 & IJBC4 & LFW \\
\midrule
FaceViT & \\
FaceCLIP-L-14 &  \\
FaceCLIP-G-14 &   \\
\bottomrule
\end{tabularx}
\caption{Face Verification Accuracy of FaceViT, FaceCLIP-L-14, and FaceCLIP-G-14.}
\label{tab:example}
\end{table}



==> tables/long_prompt_capability.tex <==
\begin{table}
\small
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
Model & Face Sim. $\uparrow$ & CLIP-T $\uparrow$  & FID $\downarrow$ \\
\midrule
InstantID & \\
PuLID & \\
FaceCLIP-SDXL$^{\spadesuit}$ &   \\
\bottomrule
\end{tabular}
\caption{Performance on long text prompts.}
\label{tab:example}
\end{table}


